Finite Type Invariants of Links with Fixed Linking Matrix

In this paper we introduce two theories of finite type invariants for framed links with fixed linking matrix. We show that these thepries are related to the theory of Vassiliev invariants of framed links. We also study the corresponding spaces of ``chord diagrams''.

==> draws/figure40d.tex <==
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(5791,2281)(0,-10)
\put(533,1733){\ellipse{1050}{1050}}
\put(2333,1733){\ellipse{1050}{1050}}
\put(1358,533){\ellipse{1050}{1050}}
\put(4620,1546){\ellipse{1126}{1126}}
\put(5258,1508){\ellipse{1050}{1050}}
\dashline{60.000}(1058,1808)(1808,1808)
\dashline{60.000}(983,1433)(1958,1433)
\dashline{60.000}(1133,983)(1808,1583)
\dashline{60.000}(1733,833)(2108,1208)
\spline(4883,1583)
(5108,1583)(5258,1433)
	(5333,1208)(5333,1133)
\spline(4583,1433)
(4433,1283)(4433,1058)
	(4583,758)(4883,758)(5108,908)
\put(2033,1733){\makebox(0,0)[lb]{\smash{{{\rm 1+$}}}}}
\put(2108,1433){\makebox(0,0)[lb]{\smash{{{\rm 1-$}}}}}
\put(1058,758){\makebox(0,0)[lb]{\smash{{{\rm 2+$}}}}}
\put(2033,758){\makebox(0,0)[lb]{\smash{{{\rm 2-$}}}}}
\end{picture}
}

